MambaByte: Token-free Selective State Space Model

Token-free language models learn directly from raw bytes and remove the inductive bias of subword tokenization. Operating on bytes, however, results in significantly longer sequences. In this setting, standard autoregressive Transformers scale poorly as the effective memory required grows with sequence length. The recent development of the Mamba state space model (SSM) offers an appealing alternative approach with a fixed-sized memory state and efficient decoding. We propose MambaByte, a token-free adaptation of the Mamba SSM trained autoregressively on byte sequences. In terms of modeling, we show MambaByte to be competitive with, and even to outperform, state-of-the-art subword Transformers on language modeling tasks while maintaining the benefits of token-free language models, such as robustness to noise. In terms of efficiency, we develop an adaptation of speculative decoding with tokenized drafting and byte-level verification. This results in a $2.6\times$ inference speedup to the standard MambaByte implementation, showing similar decoding efficiency as the subword Mamba. These findings establish the viability of SSMs in enabling token-free language modeling.

==> config/commands.tex <==
% authors: Tushaar Gangavarapu
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: Theorems, from ICML 2024 template
% \theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: same "thanks"
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: verbatim
\makeatletter
\newcommand{\verbatimfont}[1]{\def\verbatim@font{#1}}%
\makeatother

%-TG: \sample{filepath}
\newcommand{\sample}[1]{
    \verbatimfont{\rmfamily}
    \begin{quote}
        \verbatiminput{#1}
    \end{quote}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: \review{tg}{this is a review comment}
\newcommand{\review}[2]{\textcolor{magenta}{\MakeUppercase{#1}: #2}}
\newcommand{\update}[1]{\textcolor{cyan}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: TOC stuff
\renewcommand{\contentsname}{Appendix}

\makeatletter
\patchcmd{\l@section}% <cmd>
  {\addvspace{1.0em \@plus\p@}}% <search>
  {}% <replace>
  {}{}% <success><failure>
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: Cornell email
\newcommand{\cuemail}[1]{\href{#1@cornell.edu}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: Table rule settings
\renewcommand{\toprule}{\noalign{\hrule height 0.9pt\vspace{0.15cm}}}
\renewcommand{\midrule}{\noalign{\vspace{0.1cm}\hrule height 0.7pt\vspace{0.1cm}}}
\renewcommand{\bottomrule}{\noalign{\vspace{0.1cm}\hrule height 0.9pt\vspace{0.1cm}}}

\newcommand{\tablerule}{\noalign{\vspace{0.1cm}\hrule height 0.35pt\vspace{0.1cm}}}

%-TG: table rotated text: \multirowrotate{#rows}{rotation-degree}{text}
\newcommand{\multirowrotate}[3]{\parbox[t]{2mm}{\multirow{#1}{*}{\rotatebox[origin=c]{#2}{#3}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: Big-O notation
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\bigotilde}{\widetilde{\mathcal{O}}}  %-TG: log-linear, etc.

%-TG: Identity matrix
\newcommand{\I}{\mathrm{I}}

%-TG: supports: \R, \R[n], \R[n][n]
\makeatletter
\DeclareDocumentCommand{\R}{O{} O{}}{
    \ifx&#1&\@empty\relax {
        \ifx&#2&\@empty\relax {
            \mathbb{R}
        } \else {
            \mathbb{R}^{#2}
        }
        \fi
    } \else {
        \ifx&#2&\@empty\relax {
            \mathbb{R}^{#1}
        } \else {
            \mathbb{R}^{#1 \times #2}
        }
        \fi
    } 
    \fi
}
\makeatother

%-TG: Derivative in Leibniz notation
\DeclareMathOperator{\dd}{d}
\newcommand{\ddt}[1]{\frac{{\dd}#1}{{\dd}t}}
\newcommand{\dt}{{\dd}t}  %-TG: "dt"
\newcommand{\dv}{{\dd}v}  %-TG: "dv"

%-TG: "discrete" operator notation; https://latex.org/forum/viewtopic.php?t=15978
\newcommand{\discrete}[1]{
    \vbox{%
        \hrule height 0.55pt  %-TG: line above with certain width
        \kern0.3ex  %-TG: distance b/w line and content
        \hbox{%
            \kern-0.0em  %-TG: distance b/w content and left side of box
            \ifmmode#1\else\ensuremath{#1}\fi  %-TG: the content, typeset in dependence of mode
            \kern-0.0em  %-TG: distance b/w content and right side of box
        }
    }
}

%-TG: A, B, C, D matrices
\DeclareMathOperator{\A}{\mathrm{A}}
\DeclareMathOperator{\B}{\mathrm{B}}
\DeclareMathOperator{\C}{\mathrm{C}}
\DeclareMathOperator{\D}{\mathrm{D}}

%-TG: Linear; \linear{weight_id}{x}
\newcommand{\linear}[2]{W_{#1}#2}
\DeclareMathOperator{\softplus}{softplus}

%-TG: Bits Per Byte (BPB), perplexity (PPL)
\DeclareMathOperator{\bpb}{BPB}
\DeclareMathOperator{\ppl}{PPL}

%-TG: Vandermonde matrix
\DeclareSymbolFont{matha}{OML}{txmi}{m}{it}
\DeclareMathSymbol{\varv}{\mathord}{matha}{118}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: SSM name variable
\newcommand{\ssmname}{MambaByte\xspace}

\newcommand{\smallssmlayers}{$53$}
\newcommand{\smallssmsize}{$353$M}
\newcommand{\smallssmdim}{$1,024$}
\newcommand{\smallssmexp}{$2$}
\newcommand{\smallssm}{\ssmname-\smallssmsize\xspace}
\newcommand{\smallssmconfig}{%
    $n = \text{\smallssmlayers}$,
    $d = \text{\smallssmdim}$,
    $e = \text{\smallssmexp}$%
}

\newcommand{\mediumssmsize}{$972$M}
\newcommand{\mediumssmdim}{$1,792$}
\newcommand{\mediumssmexp}{$2$}
\newcommand{\mediumssmlayers}{$48$}
\newcommand{\mediumssm}{\ssmname-\mediumssmsize\xspace}
\newcommand{\mediumssmconfig}{%
    $n = \text{\mediumssmlayers}$,
    $d = \text{\mediumssmdim}$,
    $e = \text{\mediumssmexp}$%
}

\newcommand{\bigssmsize}{$1.6$B}
\newcommand{\bigssmdim}{$2,304$}
\newcommand{\bigssmexp}{$2$}
\newcommand{\bigssmlayers}{$48$}
\newcommand{\bigssm}{\ssmname-\bigssmsize\xspace}
\newcommand{\bigssmconfig}{%
    $n = \text{\bigssmlayers}$,
    $d = \text{\bigssmdim}$,
    $e = \text{\bigssmexp}$%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\megabytesmall}{MegaByte-$758$M+$262$M\xspace}
\newcommand{\megabytemedium}{MegaByte-$1.3$B+$218$M\xspace}
\newcommand{\megabytelarge}{MegaByte-$1.3$B+$350$M\xspace}
\newcommand{\megabyteours}{MegaByte-$193$M+$177$M\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: "free" footnote for version history.
\let\svthefootnote\thefootnote
\newcommand\freefootnote[1]{%
  \let\thefootnote\relax%
  \footnotetext{#1}%
  \let\thefootnote\svthefootnote%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: no-fill comment
\algnewcommand{\LeftComment}[1]{~~~~\textcolor{darkgreen}{\(\triangleright\) #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: floatrow commands
\newfloatcommand{capbtabbox}{table}[][\FBwidth]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> config/imports.tex <==
% authors: Tushaar Gangavarapu
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: colors
\usepackage{color}
\usepackage{xcolor}

\definecolor{darkblue}{rgb}{0, 0, 0.5}
\definecolor{darkgreen}{rgb}{0, 0.5, 0}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{booktabs}
\usepackage[
    colorlinks,
    linkcolor=darkblue,
    citecolor=darkblue,
    linkcolor=darkblue,
    urlcolor=darkblue
]{hyperref}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{url}
\usepackage{amsfonts}
\usepackage{nicefrac}
\usepackage{latexsym}
\usepackage{array}
\usepackage{multirow}
\usepackage{alltt}
\usepackage{enumerate}
\usepackage{bbm}
\usepackage{eucal}
\usepackage{xspace}
\usepackage{stmaryrd}
\usepackage{bussproofs}
\usepackage{mathpartir}
\usepackage{tikz}
\usepackage{pgfmath}
\usepackage{xurl}
\usepackage{mdframed}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{listings}
\usepackage{xparse}
\usepackage{xifthen}
\usepackage{multicol}
\usepackage{xfrac}
\usepackage{appendix}
\usepackage{etoolbox}
\usepackage{floatflt}
\usepackage{wrapfig}
\usepackage{tablefootnote}
\usepackage{makecell}
\usepackage{verbatim}
\usepackage{setspace}
\usepackage{floatrow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: algorithm
\usepackage{algorithm}
\usepackage[%
    noEnd=true,%
    indLines=true,%
    italicComments=false,%
    commentColor=darkgreen,%
]{algpseudocodex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%-TG: better spacing: http://tex.stackexchange.com/questions/172702/how-can-i-make-lstlisting-look-exactly-like-verbatim
\lstset{basicstyle=\ttfamily,columns=flexible}
\captionsetup[table]{skip=8pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> pages/appendices/d_parallel_scans.tex <==
\section{Parallel scan for linear recurrences}
\label{app:scans}

The parallelization of scan operations has been well explored \cite{ladner1980parallel,lakshmivarahan1994parallel,blelloch1990prefix}, with several scientific computing libraries containing optimized routines. In this section, we detail the use of a parallel scan for linear recurrence in $\S\ref{sec:model}$ as a specific application of a more generalized setting in $\S1.4$ of \citet{blelloch1990prefix}.

To compute a linear recurrence $h[k] = \discrete{A}h[k-1] + \discrete{B}x[k]$ for a sequence of length $L$, let us define $L$ initial elements $e_{1:L}$, such that:
\begin{align}
\label{eq:scan-init}
    e_k = \left(A_k, b_k\right) \coloneqq \left(\discrete{A}, \discrete{B}x[k]\right),
\end{align}
where $A_k, \discrete{A} \in \R[n][n]$, $\discrete{B} \in \R[n][1]$, and $x[k], b_k \in \R[n]$. These initial $L$ elements are precomputed before the scan.

Now, the binary associative operator $\bullet$ to use on the linear recurrence is defined as:
\begin{align}
    \label{eq:recurrence-operator}
    e_j \bullet e_k \equiv (A_k A_j, A_k b_j + b_k).
\end{align}

\paragraph{Associativity of the operator.} Note that the binary operator shown above in (\ref{eq:recurrence-operator}) is associative:
\begin{align*}
    e_i \bullet (e_j \bullet e_k) &= e_i \bullet (A_kA_j, A_kb_j + b_k) \\
    &= ((A_kA_j)A_i, A_kA_jb_i + (A_kb_j + b_k)) \\
    &= (A_k(A_jA_i), A_k(A_jb_i + b_j) + b_k) \\
    &= (A_jA_i, A_jb_i + b_j) \bullet e_k \\
    &= (e_i \bullet e_j) \bullet e_k.
\end{align*}

\paragraph{Illustration of linear recurrence using the operator.} Using the binary associative operator in (\ref{eq:recurrence-operator}), we can see how the linear recurrence $h[k] = \discrete{A}h[k-1] + \discrete{B}x[k]$ can be computed. By setting $h[0] = 0$, we have:
\begin{align*}
    h[1] &= \discrete{B}x[1]; \\
    h[2] &= \discrete{A}\discrete{B}x[1] + \discrete{B}x[2]; \\
    h[3] &= \discrete{A}^2\discrete{B}x[1] + \discrete{A}\discrete{B}x[2] + \discrete{B}x[3]; \\
     &\vdots \\
    h[k] &= \discrete{A}^{k-1}\discrete{B}x[1] + \discrete{A}^{k-2}\discrete{B}x[2] + \dots + \discrete{A}\discrete{B}x[k-2] + \discrete{B}x[k-1].
\end{align*}

\begin{algorithm}[!ht]
    \begin{algorithmic}
        \Procedure{Reduce}{$[e_1, e_2, \dotsc, e_L]$, $\bullet$}
            \For{$d = 1, \dotsc, \log_2(L)$}
                \For{$i = 1, \dotsc, L$ in increments of $2^d$ \textbf{in parallel}}
                    \State $k \gets i + 2^d - 1$; $j \gets i + 2^{d - 1} - 1$ 
                    \State $e_k \gets e_j \bullet e_k$
                \EndFor
            \EndFor
        \EndProcedure
        \\
        \Procedure{DownSweep}{$[e_1, e_2, \dotsc, e_L]$, $\bullet$}
            \State {$e_L \gets (\I, 0)$}
            \For{$d = \log_2(L), \dotsc, 1$}
                \For{$i = 1, \dotsc, L$ in increments of $2^d$ \textbf{in parallel}}
                    \State $k \gets i + 2^d - 1$; $j \gets i + 2^{d - 1} - 1$
                    \State $\text{temp} \gets e_j$
                    \State $e_j \gets e_k$
                    \State $e_k \gets e_k \bullet \text{temp}$
                \EndFor
            \EndFor
        \EndProcedure
        \\
        \Procedure{Scan}{$[e_1, e_2, \dotsc, e_L]$, $\bullet$}
            \State $\textsc{Reduce}([e_1, e_2, \dotsc, e_L], \bullet)$ \Comment{$L - 1$ $\bullet$ computes.}
            \State $\text{all\_reduced\_out} \gets e_L$ \Comment{Last element of the inclusive scan.}
            \State $\textsc{UpSweep}([e_1, e_2, \dotsc, e_L], \bullet)$ \Comment{$L - 1$ $\bullet$ computes, $L - 1$ swaps.}
            \State \Return $[e_2, \dotsc, e_L, \text{all\_reduced\_out}]$ \Comment{Shift one to the left, append all-reduced output.}
        \EndProcedure
    \end{algorithmic}
    \caption{Blelloch work-efficient parallel (inclusive) scan on a PRAM (for an array of $L$ elements, using a binary operator $\bullet$).}
    \label{alg:scan}
\end{algorithm}

Blelloch work-efficient parallel scan \cite{blelloch1990prefix} for a given array of $L$ elements $e_{1:L}$ using the binary operator in (\ref{eq:recurrence-operator}) is shown in Algorithm~\ref{alg:scan}. We initialize $e_{1:L}$ using (\ref{eq:scan-init}) and run a parallel scan in Algorithm~\ref{alg:scan}. For illustrative purposes, let $L = 4$; now we run the reduce phase as follows:
\begin{align*}
    e_1 &= (\discrete{A}, \discrete{B}x[1]). \\
    e_2 &\gets e_1 \bullet e_2 = (\discrete{A}, \discrete{B}x[1]) \bullet (\discrete{A}, \discrete{B}x[2]) = (\discrete{A}^2, \discrete{A}\discrete{B}x[1] + \discrete{B}x[2]). \\
    e_3 &= (\discrete{A}, \discrete{B}x[3]). \\
    e_4 &\gets e_2 \bullet (e_3 \bullet e_4) \\
    &= e_2 \bullet ((\discrete{A}, \discrete{B}x[3]) \bullet (\discrete{A}, \discrete{B}x[4])) \\
    &=  (\discrete{A}^2, \discrete{A}\discrete{B}x[1] + \discrete{B}x[2]) \bullet (\discrete{A}^2, \discrete{A}\discrete{B}x[3] + \discrete{B}x[4]) \\
    &= (\discrete{A}^4, \discrete{A}^3\discrete{B}x[1] + \discrete{A}^2\discrete{B}x[2] + \discrete{A}\discrete{B}x[3] + \discrete{B}x[4]).
\end{align*}

Next, we store $e_4$ above (as all-reduced output) for later, then set $e_4 = (\I, 0)$ and run the down sweep phase as follows:
\begin{align*}
    e_2 \gets (\I, 0)&; e_4 \gets (\I, 0) \bullet (\discrete{A}^2, \discrete{A}\discrete{B}x[1] + \discrete{B}x[2]) = (\discrete{A}^2, \discrete{A}\discrete{B}x[1] + \discrete{B}x[2]). \\
    e_1 \gets (\I, 0)&; e_2 \gets (\I, 0) \bullet (\discrete{A}, \discrete{B}x[1]) = (\discrete{A}, \discrete{B}x[1]). \\
    e_3 \gets (\discrete{A}^2, \discrete{A}\discrete{B}x[1] + \discrete{B}x[2])&; e_4 \gets (\discrete{A}^2, \discrete{A}\discrete{B}x[1] + \discrete{B}x[2]) \bullet (\discrete{A}, \discrete{B}x[3]) \\
    &\phantom{;  e_4   ~} = (\discrete{A}^3, \discrete{A}^2\discrete{B}x[1] + \discrete{A}\discrete{B}x[2] + \discrete{B}x[3]).
\end{align*}

To generate an inclusive scan, we shift the resulting array one to the left and insert the all-reduced output to the end. As a result, we have the output elements of the parallel scan, $r_{1:4}$, as:
\begin{align*}
    r_1 &= e_2 = (\discrete{A}, \discrete{B}x[1]) = (\discrete{A}, h[1]); \\
    r_2 &= e_3 = (\discrete{A}^2, \discrete{A}\discrete{B}x[1] + \discrete{B}x[2]) = (\discrete{A}^2, h[2]); \\
    r_3 &= e_4 = (\discrete{A}^3, \discrete{A}^2\discrete{B}x[1] + \discrete{A}\discrete{B}x[2] + \discrete{B}x[3]) = (\discrete{A}^3, h[3]); \\
    r_4 &= (\discrete{A}^4, \discrete{A}^3\discrete{B}x[1] + \discrete{A}^2\discrete{B}x[2] + \discrete{A}\discrete{B}x[3] + \discrete{B}x[4]) = (\discrete{A}^4, h[4]).
\end{align*}

Observe that the second entry $b_k$ of $r_k = (A_k, b_k)$ corresponds to the desired $h[k]$. 

\paragraph{Efficiency of a parallel scan.} From Algorithm~\ref{alg:scan}, we note that the scan operation can be performed in $\bigo(T_\bullet\log_2(L))$ time using $L/2$ processors, where $T_\bullet$ is the cost of computing $e_j \bullet e_k$. $T_\bullet$ depends on the structure of $\discrete{A}$; for a general $\discrete{A}$, $T_\bullet$ is dominated by the cost of matrix-matrix multiplication, $\bigo(n^3)$. Hence, the overall cost of a parallel scan for an $L$-length sequence and a general $\discrete{A}$ is $\bigo(n^3 \log_2(L))$.

Furthermore, for $F_\bullet$ FLOPs per $\bullet$ compute, we note the parallel scan to incur $\bigo(F_\bullet L)$ FLOPs, making the work-efficient parallel scan theoretically efficient for a tractable $F_\bullet$. For a general $\discrete{A}$, Algorithm~\ref{alg:scan} results in $\bigo(n^3 L)$ FLOPs.
